Popcorn: Accelerating Kernel K-means on GPUs through Sparse Linear Algebra

K-means is a popular clustering algorithm with significant applications in numerous scientific and engineering areas. One drawback of K-means is its inability to identify non-linearly separable clusters, which may lead to inaccurate solutions in certain cases. Kernel K-means is a variant of classical K-means that can find non-linearly separable clusters. However, it scales quadratically with respect to the size of the dataset, taking several minutes to cluster even medium-sized datasets on traditional CPU-based machines. In this paper, we present a formulation of Kernel K-means using sparse-dense matrix multiplication (SpMM) and sparse matrix-vector multiplication (SpMV), and we show that our formulation enables the rapid implementation of a fast GPU-based version of Kernel K-means with little programming effort. Our implementation, named Popcorn, is the first open-source GPU-based implementation of Kernel K-means. Popcorn achieves a speedup of up to 123.8x over a CPU implementation of Kernel K-means and a speedup of up to 2.6x over a GPU implementation of Kernel K-means that does not use sparse matrix computations. Our results support the effectiveness of sparse matrices as tools for efficient parallel programming.

==> Extra.tex <==
\section*{Attachments}
\subsection*{Distances matrix multiplication examples}
\begin{multicols}{2}
\textbf{1D example}
\begin{align*}
    c=(7),\quad p_1=(3), p_2=(1)
\end{align*}
Using directly \eqref{eq:eucl_dist} we have:
\begin{align*}
    dist^2(p_1,c) & =(3-7)^2=\textbf{16}\\
    dist^2(p_2,c) & =(1-7)^2=\textbf{36}
\end{align*}
We now use the new approach:
\begin{align*}
    C=\begin{bmatrix}
    47 & -7 \\
    -7 &  1 \\
    \end{bmatrix},\quad
    q_1=\begin{bmatrix}1 & 3\end{bmatrix},
    q_2=\begin{bmatrix}1 & 1\end{bmatrix}
\end{align*}
\begin{align*}
    dist^2(p_1,c) & = q_1\cdot C\cdot q_1^T \\
    & = \begin{bmatrix}1 & 3\end{bmatrix}\cdot
        \begin{bmatrix}
        49 & -7 \\
        -7 &  1 \\
        \end{bmatrix}\cdot
        \begin{bmatrix}
        1 \\
        3 \\
        \end{bmatrix} \\
    & = \begin{bmatrix}28 & -4\end{bmatrix}\cdot
        \begin{bmatrix}
        1 \\
        3 \\
        \end{bmatrix} \\
    & = 28-12 = \textbf{16}
\end{align*}
\begin{align*}
    dist^2(p_2,c) & = q_2\cdot C\cdot q_2^T \\
    & = \begin{bmatrix}1 & 1\end{bmatrix}\cdot
        \begin{bmatrix}
        49 & -7 \\
        -7 &  1 \\
        \end{bmatrix}\cdot
        \begin{bmatrix}
        1 \\
        1 \\
        \end{bmatrix} \\
    & = \begin{bmatrix}42 & -6\end{bmatrix}\cdot
        \begin{bmatrix}
        1 \\
        1 \\
        \end{bmatrix} \\
    & = 42 - 6 = \textbf{36}
\end{align*}


% \columnbreak
\textbf{2D example}
\begin{align*}
c=(1,4),\quad p=(5,2)
\end{align*}
Using directly \eqref{eq:eucl_dist} we have:
\begin{align*}
    dist^2(p,c) & =(5-1)^2 + (2-4)^2=\textbf{20}
\end{align*}
We now use the new approach:
\begin{align*}
    C=\begin{bmatrix}
    17 & -1 & -4 \\
    -1 &  1 &  0 \\
    -4 &  0 &  1 \\
    \end{bmatrix},\quad
    q=\begin{bmatrix}1 & 5 & 2\end{bmatrix}
\end{align*}
\begin{align*}
    dist^2(p_1,c) & = q_1\cdot C\cdot q_1^T \\
    & = \begin{bmatrix}1 & 5 & 2\end{bmatrix}\cdot
        \begin{bmatrix}
        17 & -1 & -4 \\
        -1 &  1 &  0 \\
        -4 &  0 &  1 \\
        \end{bmatrix}\cdot
        \begin{bmatrix}
        1 \\
        5 \\
        2 \\
        \end{bmatrix} \\
    & = \begin{bmatrix}4 & 4 & -2\end{bmatrix}\cdot
        \begin{bmatrix}
        1 \\
        5 \\
        2 \\
        \end{bmatrix} \\
    & = 4+20-4 = \textbf{20}
\end{align*} 

\textbf{3D example}
\begin{align*}
c=(5,2,3),\quad p=(4,3,2)
\end{align*}
Using directly \eqref{eq:eucl_dist} we have:
\begin{align*}
    dist^2(p,c) & =(4-5)^2 + (3-2)^2 + (2-3)^2=\textbf{3}
\end{align*}
We now use the new approach:
\begin{align*}
    C=\begin{bmatrix}
    38 & -5 & -2 & -3 \\
    -5 &  1 &  0 &  0 \\
    -2 &  0 &  1 &  0 \\
    -3 &  0 &  0 &  1 \\
    \end{bmatrix},\quad
    q=\begin{bmatrix}1 & 4 & 3 & 2\end{bmatrix}
\end{align*}
\begin{align*}
    dist^2(p_1,c) & = q_1\cdot C\cdot q_1^T \\
    & = \begin{bmatrix}1 & 4 & 3 & 2\end{bmatrix}\cdot
        \begin{bmatrix}
        38 & -5 & -2 & -3 \\
        -5 &  1 &  0 &  0 \\
        -2 &  0 &  1 &  0 \\
        -3 &  0 &  0 &  1 \\
        \end{bmatrix}\cdot
        \begin{bmatrix}
        1 \\
        4 \\
        3 \\
        2 \\
        \end{bmatrix} \\
    & = \begin{bmatrix}6 & -1 & 1 & -1\end{bmatrix}\cdot
        \begin{bmatrix}
        1 \\
        4 \\
        3 \\
        2 \\
        \end{bmatrix} \\
    & = 6-4+3-2 = \textbf{3}
\end{align*}

\end{multicols}

\newpage

\subsection*{Split matrix multiplications in $\delta$ dim chunks}

If instead of using libraries like cuBLAS a direct approach is preferred, follows how the multiplication can be divided in sub-operations of size $\delta\times\delta$.

Let $C\in\mathbb{R}^{r\times s}$ ($r=s$ by definition of $C$, we will use only $r$) and $P\in\mathbb{R}^{q\times r}$.

Consider the multiplication $P\cdot C \cdot P^T$, we can develop this multiplication reducing the dimensionality of each sub-operation to a maximum size $\delta$. Let's set the chunk size to $\delta$, then the matrix $C$ is padded left and bottom with $\epsilon$ rows/columns of $0$s s.t. $(r + \epsilon)\ mod\ \delta = 0$, set $r\defeq r + \epsilon$.
\[\text{Let: }
\Delta r \defeq\left\lceil \frac{r}{\delta} \right\rceil, 
\Delta q \defeq\left\lceil \frac{q}{\delta} \right\rceil
\qquad C=\begin{bmatrix}
        c_{11} & c_{12} & \dots & c_{1r} \\
        c_{21} & \dots  &    &   \\
        \dots  &   & \dots&   \\
        c_{r1} &   &    &  c_{rr} \\
      \end{bmatrix}\implies
\]
\begin{equation*}
    \implies\left[ \begin{array}{cccc|ccc|c|ccc}
        c_{11} & c_{12} & \dots & c_{1\delta} & c_{1(\delta +1)} & \dots & c_{1(2\delta)} & \dots & c_{1((\Delta r-1)\delta +1)} & \dots & c_{1(\delta\Delta r)} \\
        c_{21} & \ddots & & & & & & & & & \vdots \\
        \vdots & & \ddots & & & & & & & \\
        c_{\delta 1} & & & c_{\delta\delta} & & & & & & \\
        \midrule
        c_{(\delta +1)1} & & & & & & & & &  \\
        \vdots & & & & & \ddots & & & & & \vdots \\
        c_{(2\delta)1} & & & & & & & & & \\
        \midrule
        \vdots & & & & & & & \ddots & & & \vdots \\
        \midrule
        c_{((\Delta r-1)\delta +1)1} & & & & & & & & \ddots & \\
        \vdots & & & & & & & & & \ddots & \vdots \\
        c_{(\delta\Delta r)1} & \dots & & & & \dots & & \dots & & \dots & c_{(\delta\Delta r)(\delta\Delta r)}
      \end{array}\right] =
\end{equation*}

\begin{equation}
    =\left[ \begin{array}{c|c|c|c}
        C_{11} & C_{12} & \dots & C_{1\Delta r} \\
        \midrule 
        C_{21} & \ddots  &    &   \\
        \midrule 
        \vdots  &   & \ddots &   \\
        \midrule 
        C_{\Delta r 1} &   &    &  C_{\Delta r\Delta r} \\
    \end{array}\right] = C_{chunked}
\end{equation}

Then apply the same procedure to $P$ obtaining: $\qquad P_{chunked} = \left[ \begin{array}{c|c|c|c}
        P_{11} & P_{12} & \dots & P_{1\Delta r} \\
        \midrule 
        P_{21} & \ddots  &    &   \\
        \midrule 
        \vdots  &   & \ddots &   \\
        \midrule 
        P_{\Delta q 1} &   &    &  P_{\Delta q\Delta r} \\
    \end{array}\right]$

Consider $P_{chunked}\cdot C_{chunked}\cdot P_{chunked}^T$\footnote{$P_{chunked}^T$ transposes the whole original matrix P.}, let $i$ be a parameter that identifies a row, then:
\begin{multline}\label{eq_di}
    D_{i} = [P_{i1},P_{i2},\dots,P_{i\Delta r}]\cdot C_{chunked}\cdot[P_{i1},P_{i2},\dots,P_{i\Delta r}]^T = \\
    =[P_{i1}C_{11} + P_{i2}C_{21} + \dots + P_{i\Delta r}C_{\Delta r1},\quad P_{i1}C_{12} + P_{i2}C_{22} + \dots + P_{i\Delta r}C_{\Delta r2},\dots\\
    \dots ,P_{i1}C_{1\Delta r} + P_{i2}C_{2\Delta r} + \dots + P_{i\Delta r}C_{\Delta r\Delta r}]\cdot [P_{i1}^T,P_{i2}^T,\dots,P_{i\Delta r}^T]^T
\end{multline}

Let $diag:\mathbb{R}^{r\times r}\to \mathbb{R}^r$ be the function that "extracts" the main diagonal of a matrix e.g. $diag(M)$ returns the main diagonal of the matrix $M$.
\begin{equation}
    D=\begin{bmatrix}
        diag(D_1) &  &  &  \\
         & diag(D_2)  &    &   \\
         &   & \ddots &   \\
         &   &  & diag(D_{\Delta q}) \\
    \end{bmatrix}
\end{equation}

The vector $diag(D)\in\mathbb{R}^q$ contains the distances of the points in $P$ from the center e.g. $d_{33}\equiv diag(D)_3$ is the distance of the point number $3$ from the center.

\textit{Observation:} many of the multiplications in \eqref{eq_di} can be simplified: $P_{ab}C_{ij}=0_{\delta\delta}\quad$ if $ i,j>1\wedge i\neq j\quad\forall a,b$\footnote{$0_{\delta\delta}$ denotes a matrix in $\mathbb{R}^{\delta\times\delta}$ filled with $0$s.}

\subsection*{Computational complexity}
Let $\theta_{cnk} = max(\Delta r, \Delta q)$, the overall computational complexity of the procedure is:
\begin{equation}
    O(2(\theta_{cnk}^2 - (3\theta_{cnk} + 2)))\ \text{ having } P_{ab}C_{ij} \text{ as } O(1)
\end{equation}
Let $\theta = max(r, q)$ Without chunking the complexity is:
\begin{equation}
    O(\theta^2)\text{ having } p_{ab}c_{ij} \text{ as } O(1)
\end{equation}
Since $\theta_{cnk} \defeq\left\lceil \frac{\theta}{\delta} \right\rceil$ and $P_{ab}C_{ij}$ costs $O(\delta^2)$, the two complexities are similar.

Using tensor cores, we can approximate the cost of $P_{ab}C_{ij}$ as $O(1)$, obtaining a performance improvement of $\delta^2$ w.r.t. a classical implementation of $P\cdot C\cdot P^T$.\\
\textit{Note: the matrix multiplication approach has a squared computational complexity w.r.t the warp-oriented one. Therefore same performances can be achieved only if the cost of $P_{ab}C_{ij}$ with tensor cores is similar to $p_{ab}c_{ij}$.}

\newpage

\subsection*{Tests results} \label{attach:tests}

\begin{table}[H]
  \begin{minipage}[b]{0.5\linewidth}
    \centering
    \begin{tabular}{|l|l|l|l|l|l|}
    \hline
        \multirow{2}{*}{Impl.} & \multicolumn{5}{c|}{Features} \\ \cline{2-6}
        & 2 & 3 & 10 & 35 & 256 \\ \hline
        gpu & 242us & 148us & 175us & \cellcolor{green!50}320us & \cellcolor{green!50}285us \\ \hline
        kcuda & 239ms & 31ms & 26ms & 27ms & 29ms \\ \hline
        cpu & \cellcolor{green!50}47us & \cellcolor{green!50}35us & \cellcolor{green!50}136us & 642us & 1537us \\ \hline
        sklearn & 42ms & 5ms & 5ms & 5ms & 6ms \\ \hline
        gpu\_mtx & \cellcolor{red!50}384ms & \cellcolor{red!50}200ms & \cellcolor{red!50}209ms & \cellcolor{red!50}222ms & \cellcolor{red!50}205ms \\ \hline
    \end{tabular}
    \caption{$n=10^2$, $k=4$}
  \end{minipage}%
  \begin{minipage}[b]{0.5\linewidth}
    \centering
    \begin{tabular}{|l|l|l|l|l|l|}
    \hline
        \multirow{2}{*}{Impl.} & \multicolumn{5}{c|}{Features} \\ \cline{2-6}
         & 2 & 3 & 10 & 35 & 256 \\ \hline
        gpu & 225us & 211us & \cellcolor{green!50}170us & \cellcolor{green!50}257us & \cellcolor{green!50}284us \\ \hline
        kcuda & 49ms & 27ms & 26ms & 26ms & 28ms \\ \hline
        cpu & \cellcolor{green!50}73us & \cellcolor{green!50}95us & 198us & 802us & 2ms \\ \hline
        sklearn & 14ms & 7ms & 7ms & 7ms & 9ms \\ \hline
        gpu\_mtx & \cellcolor{red!50}409ms & \cellcolor{red!50}224ms & \cellcolor{red!50}216ms & \cellcolor{red!50}224ms & \cellcolor{red!50}205ms \\ \hline
    \end{tabular}
    \caption{$n=10^2$, $k=10$}
  \end{minipage}
\end{table}

\begin{table}[H]
  \begin{minipage}[b]{0.5\linewidth}
    \centering
    \begin{tabular}{|l|l|l|l|l|l|}
    \hline
        \multirow{2}{*}{Impl.} & \multicolumn{5}{c|}{Features} \\ \cline{2-6}
        & 2 & 3 & 10 & 35 & 256 \\ \hline
        gpu & \cellcolor{green!50}160us & \cellcolor{green!50}757us & \cellcolor{green!50}1ms & \cellcolor{green!50}2ms & \cellcolor{green!50}4.5ms \\ \hline
        kcuda & 27ms & 31ms & 30ms & 32ms & 58ms \\ \hline
        cpu & 329us & 2ms & 8ms & 23ms & 93ms \\ \hline
        sklearn & 5ms & 5ms & 6ms & 7ms & 13ms \\ \hline
        gpu\_mtx & \cellcolor{red!50}392ms & \cellcolor{red!50}1.2s & \cellcolor{red!50}1.7s & \cellcolor{red!50}1.6s & \cellcolor{red!50}1.4s \\ \hline
    \end{tabular}
    \caption{$n=10^3$, $k=4$}
  \end{minipage}%
  \begin{minipage}[b]{0.5\linewidth}
    \centering
    \begin{tabular}{|l|l|l|l|l|l|}
    \hline
        \multirow{2}{*}{Impl.} & \multicolumn{5}{c|}{Features} \\ \cline{2-6}
         & 2 & 3 & 10 & 35 & 256 \\ \hline
        gpu & \cellcolor{green!50}793us & \cellcolor{green!50}1ms & \cellcolor{green!50}3,5ms & \cellcolor{green!50}10ms & \cellcolor{green!50}23ms \\ \hline
        kcuda & 29ms & 31ms & 29ms & 29ms & 43ms \\ \hline
        cpu & 14ms & 18,5ms & 58ms & 146ms & 571ms \\ \hline
        sklearn & 12,5ms & 13ms & 13,5ms & 13ms & 22ms \\ \hline
        gpu\_mtx & \cellcolor{red!50}14s & \cellcolor{red!50}14s & \cellcolor{red!50}16s & \cellcolor{red!50}13s & \cellcolor{red!50}+5min \\ \hline
    \end{tabular}
    \caption{$n=10^3$, $k=10^2$}
  \end{minipage}
\end{table}

\begin{table}[H]
  \begin{minipage}[b]{0.5\linewidth}
    \centering
    \begin{tabular}{|l|l|l|l|l|l|}
    \hline
        \multirow{2}{*}{Impl.} & \multicolumn{5}{c|}{Features} \\ \cline{2-6}
        & 2 & 3 & 10 & 35 & 256 \\ \hline
        gpu & \cellcolor{green!50}2ms & \cellcolor{green!50}3ms & \cellcolor{green!50}9ms & \cellcolor{green!50}71ms & \cellcolor{green!50}245ms \\ \hline
        kcuda & 67ms & 169ms & 161ms & 349ms & 658ms \\ \hline
        cpu & 21ms & 26ms & 130ms & 1,1s & 3,4s \\ \hline
        sklearn & 11ms & 14ms & 40ms & 74ms & 348ms \\ \hline
        gpu\_mtx & \cellcolor{red!50}14.4s & \cellcolor{red!50}15.7s & \cellcolor{red!50}28s & \cellcolor{red!50}63s & \cellcolor{red!50}69s \\ \hline
    \end{tabular}
    \caption{$n=10^4$, $k=4$}
  \end{minipage}%
  \begin{minipage}[b]{0.5\linewidth}
    \centering
    \begin{tabular}{|l|l|l|l|l|l|}
    \hline
        \multirow{2}{*}{Impl.} & \multicolumn{5}{c|}{Features} \\ \cline{2-6}
         & 2 & 3 & 10 & 35 & 256 \\ \hline
        gpu & \cellcolor{green!50}77ms & 104ms & 404ms & 1s & 3,7s \\ \hline
        kcuda & 309ms & \cellcolor{green!50}73ms & \cellcolor{green!50}71,5ms & \cellcolor{green!50}94ms & \cellcolor{green!50}566ms \\ \hline
        cpu & \cellcolor{red!50}2,5s & \cellcolor{red!50}2,6s & \cellcolor{red!50}7,3s & \cellcolor{red!50}24s & \cellcolor{red!50}102,6s \\ \hline
        sklearn & 653ms & 328ms & 358ms & 358ms & 687ms \\ \hline
        gpu\_mtx & - & - & - & - & - \\ \hline
    \end{tabular}
    \caption{$n=10^4$, $k=10^3$}
  \end{minipage}
\end{table}


\begin{table}[H]
  \begin{minipage}[b]{0.5\linewidth}
    \centering
    \begin{tabular}{|l|l|l|l|l|l|}
    \hline
        \multirow{2}{*}{Impl.} & \multicolumn{5}{c|}{Features} \\ \cline{2-6}
        & 2 & 3 & 10 & 35 & 256 \\ \hline
        gpu & \cellcolor{green!50}3,9ms & \cellcolor{green!50}68ms & \cellcolor{green!50}160ms & \cellcolor{green!50}879ms & \cellcolor{green!50}7,4s \\ \hline
        kcuda & 95ms & 3,5s & 2,5s & 7,6s & 22,2s \\ \hline
        cpu & 42ms & 961ms & 2,6s & 13,3s & 229s \\ \hline
        sklearn & 25ms & 166ms & 312ms & 666ms & 14,5s \\ \hline
        gpu\_mtx & \cellcolor{red!50}25,4s & \cellcolor{red!50}+5min & \cellcolor{red!50}+5min & \cellcolor{red!50}+5min & \cellcolor{red!50}+5min \\ \hline
    \end{tabular}
    \caption{$n=10^5$, $k=4$}
  \end{minipage}%
  \begin{minipage}[b]{0.5\linewidth}
    \centering
    \begin{tabular}{|l|l|l|l|l|l|}
    \hline
        \multirow{2}{*}{Impl.} & \multicolumn{5}{c|}{Features} \\ \cline{2-6}
         & 2 & 3 & 10 & 35 & 256 \\ \hline
         gpu & 29s & 13s & 36s & 94s & 172s \\ \hline
        kcuda & \cellcolor{green!50}3s & \cellcolor{green!50}1,8s & \cellcolor{green!50}2,9s & \cellcolor{green!50}3,6s & \cellcolor{green!50}22,5s \\ \hline
        cpu & \cellcolor{red!50}276s & \cellcolor{red!50}161s & +\cellcolor{red!50}5min & \cellcolor{red!50}+5min & \cellcolor{red!50}+5min \\ \hline
        sklearn & 29s & 34s & 32s & 24s & 34s \\ \hline
        gpu\_mtx & - & - & - & - & - \\ \hline
    \end{tabular}
    \caption{$n=10^5$, $k=10^3$}
  \end{minipage}
\end{table}

==> bib.tex <==
\begin{thebibliography}{1}

\bibitem{Yinyang}  

\end{thebibliography}
